The Role of Compositionality in Constructing Complementarity Classical Structures Within Qubit Systems

Observables in a quantum system, represented by a Hilbert space, are given by the orthogonal bases of the aforementioned Hilbert space. Categorical Quantum Mechanics provides further abstraction of such observables, allowing for a diagrammatic representation of measurements that extends to quantum processes. Our research studies this abstraction of observables, which has been dubbed as classical structures, in a subtheory of quantum mechanics which focuses on qubit systems (or 2-dimensional quantum system and its composites). We have constructed a procedure that takes the complementary classical structures of a single qubit system and compose them separably via the Kronecker product or 'entangle' them via Bell states to obtain complementary classical structures in $n$-qubit systems. In this present work, we apply our procedure to two qubit and three qubit systems as examples. Then, using rewriting rules of ZX-calculus and tools in graph theory, we searched for maximal complete sets of mutually complementary classical structures (the categorical counterpart of mutually unbiased bases) among our constructed composite classical structures. For two qubits, we found 13 maximal complete sets of mutually complementary classical structures, and for three qubits, we found 32,448 maximal complete sets of mutually complementary classical structures.

==> list/theorem-CDname.tex <==

\begin{theorem}
For any pair of classical structures $\mathcal{A}$ and $\mathcal{B}$ with names $A$ and $B$, if $A*B\in\mathsf{T}$, then $\mathcal{A}$ and $\mathcal{B}$ are complementary.
\end{theorem}
\begin{proof}
Let $\mathcal{A}$ and $\mathcal{B}$ be composite classical structures on three qubits with names:
$$A=
\begin{bmatrix}
c_1 & c_2 & c_3\\
e_{1,2} & e_{2,3} & e_{3,1}
\end{bmatrix}
\text{ and }
B=
\begin{bmatrix}
d_1 & d_2 & d_3\\
f_{1,2} & f_{2,3} & f_{3,1}
\end{bmatrix}$$ 
such that $A*B\in\mathsf{T}$. Suppose $\mathcal{A}$ and $\mathcal{B}$ are not complementary. 

We know that $A*B=$
$\begin{bmatrix}
c_1+d_1 & c_2+d_2 & c_3+d_3\\
e_{1,2}+f_{1,2} & e_{2,3}+f_{2,3} & e_{3,1}+f_{3,1}
\end{bmatrix}$
$\in\mathsf{T}$. So there must be a pair of complementary classical structures $\mathcal{A}'$ and $\mathcal{B}'$ with names $A'$ and $B'$, respectively, such that $A'*B'=A*B$. 

Let $\mathcal{D}$ and $\mathcal{D}'$ be complementary diagrams for pairs $(\mathcal{A},\mathcal{B})$ and $(\mathcal{A}',\mathcal{B}')$, respectively, and let $t_m$ and $t'_m$ be the respective slices of $\mathcal{D}$ and $\mathcal{D}'$ on the $m$-th qubit. The top-bottom constituent pair in $t_m$ can be obtained from the $m$-th entries of the first rows of $A$ and $B$, and its connecting wires to slices on other qubits can be obtained from the $(m-1)$-th and $m$-th entries of the second rows of $A$ and $B$ for $m=2,3$, and $m$-th and $(m+1)$-th entries for $m=1$. The following is the slice $t_m$:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/84-slice-name.pdf}
\end{equation*}
Above, $(p,m,q)\in\{(3,1,2),(1,2,3),(2,3,1)\}$. The labelled boxes are connecting wires corresponding to their labels, and the labelled spiders are spiders of classical structures corresponding to their labels.

Since $\mathcal{D}$ does not satisfy the complementarity condition while $\mathcal{D}'$ satisfies the complementarity condition, this means that for some $m$, $t_m\not=t'_m$. One way that this is possible is if $t_m=\had\circ t'_m\circ\had$. However, this does not affect the complementarity of the diagrams $\mathcal{D}$ and $\mathcal{D}'$. 

Another possibility is $t_m=(t_m')^\dagger$. 

Let the names of $\mathcal{A}'$ and $\mathcal{B}'$ be defined, respectively, as $A'=$
$\begin{bmatrix}
c_1'&c_2'&c_3'\\
e'_{1,2}&e'_{2,3}&e'_{3,1}
\end{bmatrix}$
and
$B'=$
$\begin{bmatrix}
d_1'&d_2'&d_3'\\
f_{1,2}'&f_{2,3}'&f_{3,1}'
\end{bmatrix}$. 
So the slice $t_m'$ of $\mathcal{D}_m'$ takes the following form:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/84-slice-name-prime.pdf}
\end{equation*}
where $(p,m,q)\in\{(3,1,2),(1,2,3),(2,3,1)\}$.

Suppose $t_m=(t_m')^\dagger$. Then
\begin{align}
   && c_m'=d_m && d_m'=c_m &&\\
   && e_{p,m}'=f_{p,m} && f_{p,m}'=e_{p,m} && \label{eq:cw-equiv-name-1}\\
  && e_{m,q}'=f_{m,q} && f_{m,q}'=e_{m,q} && \label{eq:cw-equiv-name-2}
\end{align}

If $t_p=(t_p')^\dagger$ and $t_q=(t_q')^\dagger$, then $\mathcal{D}=(\mathcal{D}')^\dagger$ which contradicts our assumption that classical structures $\mathcal{A}$ and $\mathcal{B}$ are not complementary. So either $t_p=(t_p')^\dagger$ and $t_q=t_q'$, or $t_q=(t_q')^\dagger$ and $t_p=t_p'$, or $t_p=t_p'$ and $t_q=t_q'$. The first two cases can be subsumed by the other without loss of generality.

\noindent\textbf{Case 1}: 
Suppose $t_p=(t_p')^\dagger$ and $t_q=t_q'$. Then:
\begin{align}
 e_{q,p}=f_{q,p}'&& f_{q,p}=e_{q,p}' && e_{q,p}=e_{q,p}' && f_{q,p}=f_{q,p}'\label{eq:cw-equiv-name-3}\\
 && e_{m,q}=e_{m,q}' && f_{m,q}=e_{m,q}' && \label{eq:cw-equiv-name-4}
\end{align}
Eqs. \ref{eq:cw-equiv-name-3} imply that $ e_{q,p}=f_{q,p}$, and Eqs. \ref{eq:cw-equiv-name-4} and \ref{eq:cw-equiv-name-2} imply that $e_{m,q}=f_{m,q}$. Thus, $e_{q,p}+f_{q,p}=0$ and $e_{m,q}+f_{m,q}=0$ which means that the slice $t_q$ in $\mathcal{D}$ is separable from the other two slices in the diagram and $\mathcal{D}$ is equivalent to the following diagram up to permutation:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/85-proof-uniqueness-1.pdf}
\end{equation*}
$\mathcal{D}$ satisfies the complementarity condition if and only if the following complementarity diagram on two qubits and complementarity diagram on a qubit satisfy the complementarity condition:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/85-proof-uniqueness-2.pdf}
\end{equation*}
Furthermore, since $t_m=(t_m')^\dagger$ and $t_p=(t_p')^\dagger$ and $t_q=t_q'$, $\mathcal{D}'$ is equivalent to the following diagram up to permutation:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/85-proof-uniqueness-3.pdf}
\end{equation*}
Since $\mathcal{D}'$ satisfies the complementarity condition, $sD_{2Q}$ and $sD_{1Q}$ must also satisfy the complementarity condition. Thus, $\mathcal{D}$ satisfies the complementarity condition which contradicts our assumption. 

\noindent\textbf{Case 2}: 
Suppose $t_p=t_p'$ and $t_q=t_q'$. Then:
\begin{align}
    && e_{p,m}=f_{p,m}' && f_{p,m}=e_{p,m}' && \label{eq:cw-equiv-name-5}\\
    && e_{m,q}=f_{m,q}' && f_{m,q}=e_{m,q}' && \label{eq:cw-equiv-name-6}
\end{align}
Eqs. \ref{eq:cw-equiv-name-1} and \ref{eq:cw-equiv-name-4} imply that $e_{p,m}=f_{p,m}$, and Eqs. \ref{eq:cw-equiv-name-6} and \ref{eq:cw-equiv-name-2} imply that $e_{m,q}=f_{m,q}$. 

Therefore, the slice $t_m$ in $\mathcal{D}$ is separable from the other two slices and $\mathcal{D}$ is equivalent to the following diagram up to permutation:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/85-proof-uniqueness-4.pdf}
\end{equation*}
$\mathcal{D}'$ is then equivalent to the following diagram up to permutation:
\begin{equation*}
    \includegraphics[scale=0.2]{images/76-100/85-proof-uniqueness-5.pdf}
\end{equation*}
This result is similar to that of the previous case, and we can conclude that $\mathcal{D}$ satisfies the complementarity condition, which again, is a contradiction to our assumption. 

Thus, if $A*B\in\mathsf{T}$, then $\mathcal{A}$ and $\mathcal{B}$ are complementary.
 
\end{proof}
